ANITA: Analytic Tableau Proof Assistant

This work presents the system ANITA (Analytic Tableau Proof Assistant) developed for teaching analytic tableaux to computer science students. The tool is written in Python and can be used as a desktop application, or in a web platform. This paper describes the logical system of the tool, explains how the tool is used and compares it to several similar tools. ANITA has already been used in logic courses and an evaluation of the tool is presented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2022 (ThEdu'22)\\
EPTCS 375, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.375.4}{10.4204/EPTCS.375.4}}
\pdfoutput=1

